PyCARL: A PyNN Interface for Hardware-Software Co-Simulation of Spiking Neural Network

We present PyCARL, a PyNN-based common Python programming interface for hardware-software co-simulation of spiking neural network (SNN). Through PyCARL, we make the following two key contributions. First, we provide an interface of PyNN to CARLsim, a computationally-efficient, GPU-accelerated and biophysically-detailed SNN simulator. PyCARL facilitates joint development of machine learning models and code sharing between CARLsim and PyNN users, promoting an integrated and larger neuromorphic community. Second, we integrate cycle-accurate models of state-of-the-art neuromorphic hardware such as TrueNorth, Loihi, and DynapSE in PyCARL, to accurately model hardware latencies that delay spikes between communicating neurons and degrade performance. PyCARL allows users to analyze and optimize the performance difference between software-only simulation and hardware-software co-simulation of their machine learning models. We show that system designers can also use PyCARL to perform design-space exploration early in the product development stage, facilitating faster time-to-deployment of neuromorphic products. We evaluate the memory usage and simulation time of PyCARL using functionality tests, synthetic SNNs, and realistic applications. Our results demonstrate that for large SNNs, PyCARL does not lead to any significant overhead compared to CARLsim. We also use PyCARL to analyze these SNNs for a state-of-the-art neuromorphic hardware and demonstrate a significant performance deviation from software-only simulations. PyCARL allows to evaluate and minimize such differences early during model development.

==> sections/spinemap.tex <==
In this section we describe how \tech{} uses the cycle-accurate simulator to generate an efficient mapping of an SNN model to the neuromorphic hardware.

\subsection{Mapping SNNs to Hardware}
We develop a design space exploration (DSE) framework within \tech{} 
involving mapping of SNNs to hardware to optimize the performance metrics in \textcolor{blue}{\texttt{snn.hw.out}}. Figure~\ref{fig:dse_overview} shows the high-level overview of the DSE framework consisting of two key steps: SNN partitioning and SNN placement. We now describe these steps in details.


\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.79\columnwidth]{images/dse.pdf}}
	\caption{Design space exploration framework in \tech{}.}
	\vspace{-10pt}
	\label{fig:dse_overview}
\end{figure}

\subsection{Implementation of SNN Partitioning}
SNNs of realistic applications have many neurons with
many synapses per neuron. As an example, the handwritten
digit recognition application needs 894 neurons to achieve
recognition accuracy of 89\% \cite{diehl2015unsupervised}. To execute this application on the neuromorphic hardware, the SNN first needs to be partitioned into clusters of neurons and synapses, where the intra-cluster \emph{local synapses} are mapped within the crossbars, and the inter-cluster \emph{global synapses} are mapped on the shared interconnect. Figure \ref{fig:cluster_demo} illustrates the clustering of an SNN model into local and global synapses.

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.5\columnwidth]{images/clustering.pdf}}
	\caption{SNN partitioned into local and global synapses.}
	\label{fig:cluster_demo}
\end{figure}

\tech{} has modular structure to incorporate different optimization algorithms for clustering. For instance, our prior work \cite{das2018mapping} implements an instance of particle-swarm optimization (PSO) \cite{kennedy2010particle}, a meta-heuristic approach to minimize the total number of spikes on global synapses. Our prior work \cite{balaji2019mapping} implements a greedy approach, roughly based on the Kernighan-Lin Graph Partitioning algorithm \cite{kernighan1970efficient} to partition SNNs, minimizing the total number of global spikes.

\tech{} can be extended with minimal efforts to implement other optimization techniques for SNN partitioning.

\subsection{Implementation of SNN Placement}
Once a SNN model is partitioned, the next step is to place the clusters on the hardware. Figure \ref{fig:cluster_placement} illustrates two alternative strategies for placing the clustered SNN model to the neuromorphic hardware. We abstract the local synapses inside each cluster. We indicate the total spikes communicated on a global synapse between two clusters as a number on the corresponding edge.

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.79\columnwidth]{images/placement.pdf}}
	\caption{Illustrating the impact of different placements of clusters of a partitioned SNN on a neuromorphic hardware.}
	\label{fig:cluster_placement}
\end{figure}

 
In the top sub-figure of Figure \ref{fig:cluster_placement}, the three clusters A, B, and C are mapped to crossbars at coordinates (1,1), (0,0), and (2,2), respectively. In the best case (with no spike traffic related rerouting), a maximum of 4 interconnect segments will be used, which we illustrate in the figure. 
In the bottom sub-figure of Figure \ref{fig:cluster_placement}, the three clusters A, B, and C are mapped to crossbars at coordinates (0,1), (0,0), and (0,2), respectively. In the best case, a maximum of two interconnect segments are used. This reduction in the number of utilized segments reduces the energy consumption on the interconnect and spike latency, which improves the application accuracy. However, this placement increase spike congestion, which can negatively impact spike latency, and hence, the application accuracy. It is clear that cluster placement is not a trivial problem. 

\tech{} implements the placement optimization algorithm as a module that can be called from the top SystemC header of NOXIM. Our previous work \cite{balaji2019mapping} implement PSO to find a cluster placement that minimizes the latency and energy consumption of the hardware. 

\tech{} users can implement any other optimization heuristics to solve the partitioning and placement problems.
Additionally, they can also optimize any combination of the performance metrics in Table \ref{tab:snn_hw_out} or implement new metrics specific to their design needs. \tech{} provides a comprehensive platform to perform these design space explorations.

\subsection{Generating Output \textcolor{blue}{\texttt{snn.map.out}}}
To define the output generated in the DSE step, we define \ineq{N_n} to be the number of neurons in the SNN and \ineq{N_c} to be the number of crossbars in the hardware.
The output \textcolor{blue}{\texttt{snn.map.out}} of \tech{} generates mapping of the SNN to the hardware, optimizing one of the performance metrics of Table \ref{tab:snn_hw_out}. This mapping is represented by the matrix \ineq{\mathcal{M} \in \mathbb{R}^{N_n\times N_c}} defined as
\begin{equation}
    \label{eq:mapping}
    \footnotesize m_{ij}\in \mathcal{M} = \begin{cases}
    1 & \text{if neuron } i \text{ is mapped to crossbar } j\\
    0 & \text{otherwise}
    \end{cases}
\end{equation}
